Sublinear Time Algorithm for Online Weighted Bipartite Matching

Online bipartite matching is a fundamental problem in online algorithms. The goal is to match two sets of vertices to maximize the sum of the edge weights, where for one set of vertices, each vertex and its corresponding edge weights appear in a sequence. Currently, in the practical recommendation system or search engine, the weights are decided by the inner product between the deep representation of a user and the deep representation of an item. The standard online matching needs to pay $nd$ time to linear scan all the $n$ items, computing weight (assuming each representation vector has length $d$), and then deciding the matching based on the weights. However, in reality, the $n$ could be very large, e.g. in online e-commerce platforms. Thus, improving the time of computing weights is a problem of practical significance. In this work, we provide the theoretical foundation for computing the weights approximately. We show that, with our proposed randomized data structures, the weights can be computed in sublinear time while still preserving the competitive ratio of the matching algorithm.

==> conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}


==> other.tex <==
\section{Other projects}

\begin{itemize}
     \item \textbf{A (Slightly) Improved Approximation Algorithm
for Metric TSP}\cite{kkg21} \href{https://arxiv.org/pdf/2007.01409.pdf}{[arxiv link]}, this paper gives $(3/2-10^{-36})$ metric TSP algorithm.
    \item \textbf{Dynamic Minimum Spanning Forest with Subpolynomial
Worst-case Update Time}\cite{nswn17} \href{https://arxiv.org/pdf/1708.03962.pdf}{[arxiv link]}, this paper gives a dynamic data structure which maintains a minimal spanning forest undergoing edge insertions and deletions with update time $O(n^{o(1)})$.
\end{itemize}

\subsection{Dynamic random matching maintenance}


 
\begin{definition}[Dynamic (unweighted) random matching maintain problem]
The goal is to design a dynamic data structure (for random matching maintenance problem) to support the following operations:
\begin{itemize}
    \item \textsc{Init}$(G)$. Initialize the algorithm with an input graph $G$. After this operation, the algorithm outputs a random matching $M$ of $G$.
    \item \textsc{Insert}$(u,v)$. Insert an edge $(u,v)$ to $G$. After this operation, the algorithm outputs a random matching $M'$ of current $G$ such that $|M'\backslash M|\le o(n)$.
    \item \textsc{Delete}$(u,v)$. Delete an edge $(u,v)$ to $G$. After this operation, the algorithm outputs a random matching $M'f$ of current $G$ such that $|M'\backslash M|\le o(n)$. 
\end{itemize}
The goal is to design such a data structure with update time as small as possible.
\end{definition}

